Unsupervised Opinion Summarization as Copycat-Review Generation

Opinion summarization is the task of automatically creating summaries that reflect subjective information expressed in multiple documents, such as product reviews. While the majority of previous work has focused on the extractive setting, i.e., selecting fragments from input reviews to produce a summary, we let the model generate novel sentences and hence produce abstractive summaries. Recent progress in summarization has seen the development of supervised models which rely on large quantities of document-summary pairs. Since such training data is expensive to acquire, we instead consider the unsupervised setting, in other words, we do not use any summaries in training. We define a generative model for a review collection which capitalizes on the intuition that when generating a new review given a set of other reviews of a product, we should be able to control the "amount of novelty" going into the new review or, equivalently, vary the extent to which it deviates from the input. At test time, when generating summaries, we force the novelty to be minimal, and produce a text reflecting consensus opinions. We capture this intuition by defining a hierarchical variational autoencoder model. Both individual reviews and the products they correspond to are associated with stochastic latent codes, and the review generator ("decoder") has direct access to the text of input reviews through the pointer-generator mechanism. Experiments on Amazon and Yelp datasets, show that setting at test time the review's latent code to its mean, allows the model to produce fluent and coherent summaries reflecting common opinions.

==> content/summs/amazon/ablation_summ1.tex <==
% B003YJ5LLM

\begin{table*}
 	\footnotesize 
 	\centering
    \begin{tabular}{ | c | p{12cm} |}
    \hline
     & \multicolumn{1}{>{\centering}m{110mm}|}{Summary} \\ \hline
    Full & This is a great case for the Acer Aspire 14' laptop. It is a little snug for my laptop, but it's a nice case. I would recommend it to anyone who wants to protect their laptop.\\ \hline
    w/o $r_{\_i}$ & This is the best case for the money. The sleeve is a little too bulky but it 's nice to be able to carry it on my laptop. I recommend it to my friends.\\ \hline
    w/o $c$ &  I love this case. It is perfect for my Acer Aspire one. It is a little snug but that's why I bought it for my laptop. I love it and recommend it.\\ \hline
    w/o $z$ & This is a great case, but I had to return it. I returned it for a refund because it was damaged when I received it. The case is the only reason I gave it 4 stars instead of 5 stars because of the price.\\ \hline 
    & \multicolumn{1}{>{\centering}m{110mm}|}{Input}\\ \hline
    Review 1 & Love the design of this sleeve. When I don't have a table I use the sleeve as a mat to protect my thighs from the heat of my laptop. Wish it had a bit more padding and cushion but other than that it's a pretty carrying sleeve.\\ \hline
    Review 2 & This was bought for our teen daughter for Christmas, the only negative things about it are 1.no strap 2.no pockets, other than that it is great, but in all fairness i knew both things about it when ordered, it came in very fast, was just as described, great item for the price.\\ \hline
    Review 3 & This case fits perfectly on my 14inch hp. I disagree with the comments that talk about the smell being terrible. The smell really wasn't that strong and went away after a couple of weeks. I love the design and it was a fair price. Shipping was a little expensive though. It arrived quickly and I would buy from this seller again.\\ \hline
    Review 4 & I really enjoy the design of this case but I thought it would be lighter. When it came, it was a very dark grey which was a bummer. But the quality is good and it has a nice thick padding to protect my laptop.\\ \hline
    Review 5 & I like this case very much! It fits my Acer Aspire 14 'as a glove!!! Yes, it smells a little bit but I wouldn't say that it's so bad as mentioned in some reviews. And it's very cute too. I recommend this product to anyone.\\ \hline
    Review 6 & I BOUGHT IT FOR MY ACER 14 ', IT IS A LITTLE BIT TIGHT, BUT THE WORST WAS IT HAS HEAVY RUBBER SMELL, WHEN I LEAVE THE CASE IN MY ROOM, THE RUBBER SMELL WAS FILLED WITH THE AIR EVERYWHERE OF MY ROOM, MADE ME SICK. DON'T BUY IT.\\ \hline
    Review 7 & I have a dell inspiron 14, and the cover is a little snug. It's working well though and now I can carry my laptop in my school backpack rather than carry a separate laptop bag. I'd recommend this product, just do a bunch of research to make sure it will fit.\\ \hline
    Review 8 & I really love it! It doesn't smell a lot as some reviews say and the draw is well defined.I bought this size for a 13.3 'because my laptop will have a cover on it so I don't know how it fits for a traditional 14 inch,\\ \hline
    \end{tabular}
    \caption{Amazon summaries of the ablated model.}
    \label{table:ama_ablation_summs1}
\end{table*}

==> content/summs/amazon/front_summ1.tex <==
 % B003YJ5LLM %

\begin{table}[h!]
 	\footnotesize 
    \begin{tabular}{ | >{\centering\arraybackslash} m{1.2cm} | m{5.5cm} |}
    \hline
    Summary & \textcolor{red}{This is a great case} \textcolor{orange}{for the Acer Aspire 14' laptop}. \textcolor{cyan}{It is a little snug for my laptop}, \textcolor{red}{but it's a nice case}. \textcolor{blue}{I would recommend it to anyone who wants to protect their laptop}. \\ \hline
    Reviews & ... \textcolor{red}{great item} ... \textcolor{red}{I like this case very much!} \textcolor{orange}{It fits my Acer Aspire 14 'as a glove!!!} ...  \textcolor{blue}{I recommend this product to anyone.}...  \textcolor{orange}{I BOUGHT IT FOR MY ACER 14 '}, \textcolor{cyan}{IT IS A LITTLE BIT TIGHT} ... \textcolor{cyan}{and the cover is a little snug} ... \textcolor{blue}{I'd recommend this product} ... \textcolor{orange}{traditional 14 inch} ...\\ \hline
    % Review 1 & Love the design of this sleeve. When I don't have a table I use the sleeve as a mat to protect my thighs from the heat of my laptop. Wish it had a bit more padding and cushion but other than that it's a pretty carrying sleeve. \\ \hline
    % Review 2 & This was bought for our teen daughter for Christmas, the only negative things about it are 1.no strap 2.no pockets, other than that \textcolor{red}{it is great}, but in all fairness i knew both things about it when ordered, it came in very fast, was just as described, \textcolor{red}{great item} for the price. \\ \hline
    % Review 3 & This case fits perfectly on my 14inch hp. I disagree with the comments that talk about the smell being terrible. The smell really wasn't that strong and went away after a couple of weeks. I love the design and it was a fair price. Shipping was a little expensive though. It arrived quickly and I would buy from this seller again. \\ \hline
    % Review 4 &  I really enjoy the design of this case but I thought it would be lighter. When it came, it was a very dark grey which was a bummer. But the quality is good and it has a nice thick padding to protect my laptop.\\ \hline
    % Review 5 & \textcolor{red}{I like this case very much!} \textcolor{orange}{It fits my Acer Aspire 14 'as a glove!!!} Yes, it smells a little bit but I wouldn't say that it's so bad as mentioned in some reviews. And it's very cute too. \textcolor{blue}{I recommend this product to anyone.} \\ \hline
    % Review 6 & \textcolor{orange}{I BOUGHT IT FOR MY ACER 14 '}, \textcolor{cyan}{IT IS A LITTLE BIT TIGHT}, BUT THE WORST WAS IT HAS HEAVY RUBBER SMELL, WHEN I LEAVE THE CASE IN MY ROOM, THE RUBBER SMELL WAS FILLED WITH THE AIR EVERYWHERE OF MY ROOM, MADE ME SICK. DON'T BUY IT. \\ \hline
    % Review 7 &   I have a dell inspiron 14, \textcolor{cyan}{and the cover is a little snug}. It's working well though and now I can carry my laptop in my school backpack rather than carry a separate laptop bag. \textcolor{blue}{I'd recommend this product}, just do a bunch of research to make sure it will fit.\\ \hline
    % Review 8 & I really love it! It doesn't smell a lot as some reviews say and the draw is well defined.I bought this size for a 13.3 'because my laptop will have a cover on it so I don't know how it fits for a \textcolor{orange}{traditional 14 inch}, \\ \hline
    \end{tabular}
    \caption{An example summary produced by our system with colored content alignment. The eight input reviews are concatenated and truncated for visibility.}
    \label{table:ama_front_example_summ1}
\end{table}

==> content/summs/amazon/front_summ2.tex <==
% B00006IUVM
% red, orange, blue, cyan, green

\begin{table}[h!] 
 	\footnotesize 
    \begin{tabular}{ | >{\centering\arraybackslash} m{1.2cm} | m{5.5cm} |}
    \hline
    Summary & This is the \textcolor{red}{best steamer I have ever owned}. It is \textcolor{orange}{easy to use} and \textcolor{cyan}{easy to clean}. I have \textcolor{blue}{used it several times} and \textcolor{red}{it works great}. I \textcolor{red}{would recommend it} to anyone looking for a steamer. \\ \hline
    Reviews &  ... \textcolor{red}{Love the steamer!} ... \textcolor{red}{We cook with it every day and love it!} ... \textcolor{red}{I love this steamer} ... \textcolor{red}{Everyone in my family now has one because they are so great} ... \textcolor{orange}{easy to use} ... \textcolor{cyan}{easy to clean} ... \textcolor{red}{I love using it to make rice} ... \textcolor{orange}{makes corn on the cob and boiled eggs hassle free} ... \textcolor{orange}{I LOVE THE VERSITILITY OF THIS ITEM} ... \textcolor{red}{JUST A USEFUL ITEM TO HAVE IN THE KITCHEN} ... \textcolor{red}{I love this steamer} ... \textcolor{red}{I highly recommend it} ... \textcolor{red}{I've been very pleased with the steamer} ...  \textcolor{blue}{used it several times already} ... \textcolor{red}{I would definately recommend this product} \\\hline
    % Review 1 & I had an almost identical steamer from Black \& Decker purchased around 1985. The lid on that one finally broke and I've been looking for one like it for 2 years. Nice to see a good design hasn't been changed. \textcolor{red}{Love the steamer!} \\ \hline
    % Review 2 & I bought this one as a replacement for an old one I had. \textcolor{red}{We cook with it every day and love it!} It is the perfect size for our family. Although the picture shows it with a clear lid, the one I received in the mail had a white lid.\\ \hline
    % Review 3 &  \textcolor{red}{I love this steamer}. \textcolor{red}{Everyone in my family now has one because they are so great}. It is \textcolor{orange}{easy to use} and \textcolor{cyan}{easy to clean}. \textcolor{red}{I love using it to make rice} - \textcolor{cyan}{no more cleaning up boiled-over rice from the stove!} It also \textcolor{orange}{makes corn on the cob and boiled eggs hassle free}.\\ \hline
    % Review 4 &  THIS IS MY SECOND ONE OF THESE STEAMERS. I USED THE FIRST ONE ALMOST DAILY FOR OVER 5 YEARS. \textcolor{orange}{I LOVE THE VERSITILITY OF THIS ITEM}. MAKES EXCELLENT STEAMED SHRIMP, THE RICE IS PERFECT EVERY TIME, VEGETABLES TASTE GREAT. \textcolor{red}{JUST A USEFUL ITEM TO HAVE IN THE KITCHEN}.\\ \hline
    % Review 5 & \textcolor{red}{I love this steamer}. I use it to steam all kinds of vegetables and new potatoes. I really like the larger basket and the screen where you can put herbs or spices to flavor what you are cooking. \textcolor{red}{I highly recommend it.} \\ \hline
    % Review 6 & Sometimes I use the steamer for just one vegetable, or for rice, but it's really nice to have the separate basket when I want to steam two separate vegetables at the same time. \textcolor{red}{I've been very pleased with the steamer} and have \textcolor{blue}{used it several times already}. The instruction book in helpful too. Thank you.\\ \hline
    % Review 7 & boiling broccoli always adds a ton of water and makes it super soggy, but this is the best way to cook broccoli (and other things of course...) \textcolor{red}{I would definately recommend this product}. The only downfall is that it's pretty big and we have NO couter space, so it makes it difficult to store it and make room for it.\\ \hline
    % Review 8 & This is our second B / D steamer. The first served us well for years before the plexiglass bowl cracked and finally broke. It was impossible to find a replacement in any major chain stores. Lots of rice steamers but no small in size vegetable steamers. Amazon came through again. Thanks Jeff! \\ \hline
    \end{tabular}
    \caption{An example summary produced by our system with colored content alignment. The eight input reviews are concatenated and truncated for visibility.}
    \label{table:ama_front_example_summ2}
\end{table}

==> content/summs/amazon/lat_analysis1.tex <==
% B0006HLVCI_11768

\begin{table*}[h!]
 	\footnotesize 
 	\centering
    \begin{tabular}{ | >{\centering\arraybackslash} m{1.cm} | m{12cm} |}
    \hline
    mean $z$ & This is the best spatula I've ever used. I have used it several times now and it is holding up well. I would recommend it to anyone looking for a good quality spatula for the price.\\ \hline
    $z_1$ & This is a great product for the price . I've been using it for a few months now and it works great. I would recommend it to anyone.\\ \hline
    $z_2$ &  This is a good product. I wish it was a bit larger, but it is a good product. I would recommend it.\\ \hline
    $z_3$ &  The jar is exactly what i was looking for. It fits my oster blender perfectly. I don't have to worry about it breaking, but I'm sure it will last a long time. I'm happy with it.\\ \hline \hline 
    Rev 1 & Since i 'm using the wok on the stove top most of the time , my temps aren 't extremely hot and i don 't often need a spatula this long . When I do need one though , this one is great . I also have the shorter version and they 're great quality . I expect they will last a long time and are a good value .\\ \hline
    Rev 2 & Joyce Chen Bamboo utensils are extremely well made ! They are nothing compared to the cheap pieces of trash you find in department stores.I have full sets of metal , polymer based , and bamboo utensils . Without thinking , I find myself grabbing these before anything else.You will NOT regret buying Joyce Chen bamboo products ! ! ! Happy cooking ! ! Denille\\ \hline
    Rev 3 & I liked the Burnished Bamboo Spatula ( 18 inch ) - it is very well made , the only problem I had was with arthritis it was a little bulky to hold . But it did what they said and was very good quality . I liked the bamboo part enough to go out and buy some other bamboo utensils .\\ \hline
    Rev 4 & I have had this about 5 mos now and it is spectacular ! I abuse the poor thing on a daily basis and even toss it in the dishwasher at least once a week and after almost 6 mos it still makes perfect stir fry and curries .. fabulous for the price GET ONE !\\ \hline
    Rev 5 & I have used this spatula several times now for stir fry , and it works great . The length of the spatula will allow you to keep your hands farther away from the wok , to decrease the chance for burns . Good quality , too .\\ \hline
    Rev 6 & Perfect length for making smoking hot stir-fry without burning myself . It 's a little lighter weight than I expected , but seems durable enough . Wouldn 't put it in a dishwasher or leave it soaking , though . Very pleased with purchase .\\ \hline
    Rev 7 & Very Good Quality and it is huge , Just the thing for a big wok . After several months of use It still looks like new . I would definitely purchase this again\\ \hline
    Rev 8 & Bought in conjunction w / a cast iron wok , as a gift for my son who loves to cook . Sturdy , does the job .\\ \hline
    \end{tabular}
    \caption{Amazon summaries of the full model with sampled and mean assignment to $z$. The assignment to $c$ was fixed, and was the mean value based on the approximate posterior $q_{\phi}(c|r_1,...,r_N)$.}
    \label{table:ama_latent_analysis_summs1}
\end{table*}

==> content/summs/amazon/summs2.tex <==
% B00006IUVM

\begin{table*}[h]
 	\footnotesize 
 	\centering
    \begin{tabular}{ | >{\centering\arraybackslash} m{1.5cm} | m{12cm} |}
    \hline
    Ours & This is the best steamer I have ever owned. It is easy to use and easy to clean. I have used it several times and it works great. I would recommend it to anyone looking for a steamer.\\ \hline
    MeanSum &  I love the fact that it's a little bit smaller than I expected. It's very easy to use and the rice is very sharp. The handles are easy to clean, and the handles are easy to clean. I would recommend this product to anyone.\\ \hline
    LexRank & Love the steamer! I love this steamer. I love this steamer. This is our second B / D steamer. \\ \hline
    Gold & This steamer is an excellent product. It does wonderful when cooking rice, boiling eggs, steaming vegetables and more! It makes clean up a breeze and even has a handy screen for putting seasoning in what your cooking. Definitely a nice addition to any kitchen!\\ \hline \hline
    Rev 1 & I had an almost identical steamer from Black \& Decker purchased around 1985. The lid on that one finally broke and I've been looking for one like it for 2 years. Nice to see a good design hasn't been changed. Love the steamer! \\ \hline
    Rev 2 & I bought this one as a replacement for an old one I had. We cook with it every day and love it! It is the perfect size for our family. Although the picture shows it with a clear lid, the one I received in the mail had a white lid.\\ \hline
    Rev 3 &  I love this steamer. Everyone in my family now has one because they are so great. It is easy to use and easy to clean. I love using it to make rice - no more cleaning up boiled-over rice from the stove! It also makes corn on the cob and boiled eggs hassle free.\\ \hline
    Rev 4 &  THIS IS MY SECOND ONE OF THESE STEAMERS. I USED THE FIRST ONE ALMOST DAILY FOR OVER 5 YEARS. I LOVE THE VERSITILITY OF THIS ITEM. MAKES EXCELLENT STEAMED SHRIMP, THE RICE IS PERFECT EVERY TIME, VEGETABLES TASTE GREAT. JUST A USEFUL ITEM TO HAVE IN THE KITCHEN.\\ \hline
    Rev 5 & I love this steamer. I use it to steam all kinds of vegetables and new potatoes. I really like the larger basket and the screen where you can put herbs or spices to flavor what you are cooking. I highly recommend it. \\ \hline
    Rev 6 & Sometimes I use the steamer for just one vegetable, or for rice, but it's really nice to have the separate basket when I want to steam two separate vegetables at the same time. I've been very pleased with the steamer and have used it several times already. The instruction book in helpful too. Thank you.\\ \hline
    Rev 7 & boiling broccoli always adds a ton of water and makes it super soggy, but this is the best way to cook broccoli (and other things of course...) I would definately recommend this product. The only downfall is that it's pretty big and we have NO couter space, so it makes it difficult to store it and make room for it.\\ \hline
    Rev 8 & This is our second B / D steamer. The first served us well for years before the plexiglass bowl cracked and finally broke. It was impossible to find a replacement in any major chain stores. Lots of rice steamers but no small in size vegetable steamers. Amazon came through again. Thanks Jeff! \\ \hline
    \end{tabular}
    \caption{Amazon summaries produced by different models.}
    \label{table:ama_example_summs2}
\end{table*}

==> content/summs/amazon/summs4.tex <==
% B003YJ5LLM

\begin{table*}[h]
 	\footnotesize 
 	\centering
    \begin{tabular}{ | >{\centering\arraybackslash} m{1.5cm} | m{12cm} |}
    \hline
    Ours & This is a great case for the Acer Aspire 14 \"laptop. It is a little snug for my laptop, but it's a nice case. I would recommend it to anyone who wants to protect their laptop.\\ \hline
    MeanSum & I was looking for a cover with a small case, and this one was a great price. I was looking for a case that is not too big and not too heavy. This one is great and I love it. I would recommend this product.\\ \hline
    LexRank & Love the design of this sleeve. I BOUGHT IT FOR MY ACER 14 ', IT IS A LITTLE BIT TIGHT, BUT THE WORST WAS IT HAS HEAVY RUBBER SMELL, WHEN I LEAVE THE CASE IN MY ROOM, THE RUBBER SMELL WAS FILLED WITH THE AIR EVERYWHERE OF MY ROOM, MADE ME SICK. I really enjoy the design of this case but I thought it would be lighter. When I don't have a table I use the sleeve as a mat to protect my thighs from the heat of my laptop. \\ \hline
    Gold &  This 14' laptop sleeve has an attractive design and is made of quality materials. It has a very snug fit, so be cautious of buying it if your laptop is even slightly over 14'. The only real issue is the rubbery smell that comes with it. Overall, I would recommend this, unless you have a sensitive nose.\\ \hline \hline 
    Rev 1 & Love the design of this sleeve. When I don't have a table I use the sleeve as a mat to protect my thighs from the heat of my laptop. Wish it had a bit more padding and cushion but other than that it's a pretty carrying sleeve.\\ \hline
    Rev 2 & This was bought for our teen daughter for Christmas, the only negative things about it are 1.no strap 2.no pockets, other than that it is great, but in all fairness i knew both things about it when ordered, it came in very fast, was just as described, great item for the price.\\ \hline
    Rev 3 & This case fits perfectly on my 14inch hp. I disagree with the comments that talk about the smell being terrible. The smell really wasn't that strong and went away after a couple of weeks. I love the design and it was a fair price. Shipping was a little expensive though. It arrived quickly and I would buy from this seller again.\\ \hline
    Rev 4 & I really enjoy the design of this case but I thought it would be lighter. When it came, it was a very dark grey which was a bummer. But the quality is good and it has a nice thick padding to protect my laptop.\\ \hline
    Rev 5 & I like this case very much! It fits my Acer Aspire 14 'as a glove!!! Yes, it smells a little bit but I wouldn't say that it's so bad as mentioned in some reviews. And it's very cute too. I recommend this product to anyone.\\ \hline
    Rev 6 & I BOUGHT IT FOR MY ACER 14 ', IT IS A LITTLE BIT TIGHT, BUT THE WORST WAS IT HAS HEAVY RUBBER SMELL, WHEN I LEAVE THE CASE IN MY ROOM, THE RUBBER SMELL WAS FILLED WITH THE AIR EVERYWHERE OF MY ROOM, MADE ME SICK. DON'T BUY IT.\\ \hline
    Rev 7 & I have a dell inspiron 14, and the cover is a little snug. It's working well though and now I can carry my laptop in my school backpack rather than carry a separate laptop bag. I'd recommend this product, just do a bunch of research to make sure it will fit.\\ \hline
    Rev 8 & I really love it! It doesn't smell a lot as some reviews say and the draw is well defined.I bought this size for a 13.3 'because my laptop will have a cover on it so I don't know how it fits for a traditional 14 inch,\\ \hline
    \end{tabular}
    \caption{Amazon summaries produced by different models.}
    \label{table:ama_example_summs4}
\end{table*}

==> content/summs/yelp/front_summ1.tex <==
\begin{table}[h!]
 	\footnotesize 
 	\centering
    \begin{tabular}{ | c | p{6cm} |}
    \hline
     & \multicolumn{1}{>{\centering}m{60mm}|}{Summary} \\ \hline
    Ours & This place is the worst service I've ever had. The food was mediocre at best. The service was slow and the waiter was very rude. I would not recommend this place to anyone who wants to have a good time at this location.\\ \hline
    Gold &  I'm really not a fan of Macaroni Grill, well, at least THIS Macaroni Grill.  The staff is slow and really doesn't seem to car about providing quality service.  It took well over 30 minutes to get my food and the place wasn't even packed with people.  I ordered pizza and it didn't taste right. I think it wasn't fully cooked.  I won't be coming back. \\ \hline
    \end{tabular}
    \caption{An example summary.}
    \label{table:yelp_front_example_summ1}
\end{table}

==> content/summs/yelp/summs1.tex <==
% 1_Dg-GguWatioW4mvFQKQA

\begin{table*}
 	\footnotesize 
 	\centering
    \begin{tabular}{ | >{\centering\arraybackslash} m{1.5cm} | m{12cm} |}
    \hline
    Ours & This place is the best sushi I've had in a long time. However, the service was slow and inattentive. If you're looking for sushi, this is the place to go if you're in the area. \\ \hline
    MeanSum & Was here with my girlfriend for the first time and it was a very good experience. It's not the best sushi restaurant in town, but it's not too far from the strip. Very clean and friendly service.  I would say, this place is a little more expensive than most sushi places in Mississauga and it's a bit pricey.\\ \hline
    % MeanSum & I orderes from this place and the sushi was good. We ordered a lot of sushi dishes, but the fact that it's in a bad way (not that much) it's not too bad - it's not 24 hours so it's not too expensive! \\ \hline
    LexRank & If she really looked, she would have seen we didn't eat one sushi roll. Sushi with great mouthfeel, well-executed rice, but not a ton of flavor.I ordered the Sushi deluxe meal, which comes with 10 pieces of nigiri (fish on top of rice, which is the only sushi in Japan.) I sure hope this isn't the best sushi in Pittsburgh. I especially liked the Dragon Roll from the 8 sushis we tried here. Not sure if I hit them on an off night, but the sushi was not good. \\ \hline
    Gold & They have a long list of meals but the sushi is wonderful and top of the list for things to get. The staff is very friendly and helpful but rush around a bit . The owner is also friendly. The place itself is average to below average. \\ \hline \hline
    Rev 1 &  Great sushi and very friendly staff (even the sushi chef and owner asked how my meal was) but the SiriusXM Love station was brutal to listen to.\\ \hline
    Rev 2 & The sushis were nice. I especially liked the Dragon Roll from the 8 sushis we tried here. We tried the Dean's, Dragon, Veggie, Rock and Roll, twister, American Dream and two others. I could say the dragon and rock and roll were among my most favorite ones but the veggies was probably the least favorite. \\ \hline
    Rev 3 & We went on a surprise date to a new place.   They were totally packed and had 2 servers on. Maybe a call off and that happens. But our server could barely get to us and just dropped food and ran. If she really looked, she would have seen we didn't eat one sushi roll.  The Dean. Pureed and super fishy. The Udon Noodles seemed Way over cooked. Wine list was crap, but I wasn't expecting anything great. We left hungry and will not return because of the food. I can forgive some slow service. \\ \hline
    Rev 4 & I heard great things about this place, which is why I was really looking forward to it.  Not sure if I hit them on an off night, but the sushi was not good.  I sure hope this isn't the best sushi in Pittsburgh.  Didn't care for the atmoshphere...kind of dingy. \\ \hline
    Rev 5 &  Stunningly bad... Not sure what else to say but if you're seeking edible Japanese food run in any direction but this place.\\ \hline
    Rev 6 &  We really like this place--super friendly owner and have never a wait for a table.Reasonably priced generous sushi boats that are excellent. I despise mayo and this is the one sushi restaurant where I don't have to worry.  The house salad dressing is very good and the udon soup bowls are a perfect warmup in winter.   The green tea is made with leaves and not tea bags which is a nice change of pace.Win.\\ \hline
    Rev 7 & Sushi with great mouthfeel, well-executed rice, but not a ton of flavor.I ordered the Sushi deluxe meal, which comes with 10 pieces of nigiri (fish on top of rice, which is the only sushi in Japan.) This comes with miso soup and the common sesame ginger salad. The miso soup was flat in flavor and the salad was OK. A bit too much sweetness/acidity from the dressing.The sushi selection was predictable. Tuna, salmon, snapper, and bbq eel. The fish was very creamy in mouthfeel (excellent) but none of them impressed me in flavor except the bbq eel, which was smoky and sweet. Rice was of good execution. \\ \hline
    Rev 8 & Wonderful sushi ver much more on the traditional side. Worth checking out if you're in Pittsburgh. \\ \hline
    \end{tabular}
    \caption{Yelp summaries produced by different models.}
    \label{table:yelp_example_summs1}
\end{table*}
